Efficient Second-Order Shape-Constrained Function Fitting

We give an algorithm to compute a one-dimensional shape-constrained function that best fits given data in weighted-$L_{\infty}$ norm. We give a single algorithm that works for a variety of commonly studied shape constraints including monotonicity, Lipschitz-continuity and convexity, and more generally, any shape constraint expressible by bounds on first- and/or second-order differences. Our algorithm computes an approximation with additive error $\varepsilon$ in $O\left(n \log \frac{U}{\varepsilon} \right)$ time, where $U$ captures the range of input values. We also give a simple greedy algorithm that runs in $O(n)$ time for the special case of unweighted $L_{\infty}$ convex regression. These are the first (near-)linear-time algorithms for second-order-constrained function fitting. To achieve these results, we use a novel geometric interpretation of the underlying dynamic programming problem. We further show that a generalization of the corresponding problems to directed acyclic graphs (DAGs) is as difficult as linear programming.

==> preamble.tex <==
\makeatletter
\usepackage{amsmath,amssymb}
\usepackage{algorithm2e}
%
\usepackage{float,placeins}
%
\usepackage{hyperref}
\usepackage{mathtools}
%
%
\usepackage[dvipsnames]{xcolor}
\usepackage{mleftright}\mleftright
\usepackage{enumitem}

\usepackage{xifthen}
\newcommand{\ifarxiv}[2]{\ifthenelse{\equal{\version}{arxiv}}{#1}{#2}}
\newcommand{\ifconf}[2]{\ifthenelse{\equal{\version}{conference}}{#1}{#2}}
%

\input{ushyphex.tex} %


\ifconf{}{
	\setlength\parindent{1.5em}
	\usepackage{colonequals}
%
	\usepackage[headsepline]{scrlayer-scrpage}
	\pagestyle{scrheadings}
	\clearscrheadfoot
	\AtBeginDocument{%
		\manualmark%
		\markleft{\mytitle}%
		\automark*[section]{}%
	}
	\ohead{\pagemark}
	\ihead{\headmark}
%
	\addtokomafont{caption}{\sffamily\small}
	\addtokomafont{captionlabel}{\sffamily\textbf}
	\setcapmargin{2em}
}


%
%
%
%
	\usepackage{microtype}
%



\ifconf{
	\let\springeremail\email
}{}


%
\newcommand*\ie{\mbox{i.\hspace{.2ex}e.}}
\newcommand*\eg{\mbox{e.\hspace{.2ex}g.}}
\newcommand*\iid{\mbox{i.\hspace{.2ex}i.\hspace{.2ex}d.}\xspace}
\newcommand*\wrt{\mbox{w.\hspace{.2ex}r.\hspace{.2ex}t.}\xspace}
\newcommand*\aka{\mbox{a.\hspace{.2ex}k.\hspace{.2ex}a.}\xspace}
\newcommand*\withoutlossofgenerality{\mbox{w.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\Withoutlossofgenerality{\mbox{W.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\almostsurely{\mbox{a.\hspace{.2ex}s.}\xspace}
\newcommand*\whp{\mbox{w.\hspace{.2ex}h.\hspace{.2ex}p.}\xspace}



%

%%
%%
%%
\def\makeboxwhd#1#2#3#4{\setbox0=\hbox{#4}%
\ht0=#2%
\dp0=#3%
\wd0=#1%
\box0%
}

\newcommand*{\vcenteredhbox}[1]{\begingroup
\setbox0=\hbox{#1}\parbox{\wd0}{\box0}\endgroup}


%%
%%
\newdimen\makeboxdimen
%
\newcommand\makeboxlike[3][l]{%
\setbox0=\hbox{#2}%
\global\makeboxdimen=\wd0%
\setbox1=\hbox{\makebox[\makeboxdimen][#1]{%
\makebox[0pt][#1]{#3}%
}}%
\ht1=\ht0%
\dp1=\dp0%
\box1%
}


\newcommand\plaincenter[1]{%
	\ignorespaces%
		\mbox{}\hfill#1\hfill\mbox{}
	\unskip%
}



\newcommand{\surroundedmath}[3]{%
	\mathchoice{%
		#1{#2{#3}#2}%
	}{%
		#1{#3}%
	}{%
		#1{#3}%
	}{%
		#1{#3}%
	}%
}
\newcommand\rel[1]{\surroundedmath{\mathrel}{\:}{#1}}
\newcommand\wrel[1]{\surroundedmath{\mathrel}{\;}{#1}}
\newcommand\wwrel[1]{\surroundedmath{\mathrel}{\;\;}{#1}}
\newcommand\bin[1]{\surroundedmath{\mathbin}{\:}{#1}}
\newcommand\wbin[1]{\surroundedmath{\mathbin}{\;}{#1}}
\newcommand\wwbin[1]{\surroundedmath{\mathbin}{\;\;}{#1}}

\newcommand{\eqwithref}[2][c]{%
	\relwithref[#1]{#2}{=}%
}
\newcommand{\relwithref}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize\wref{#2}}}}{#3}}%
}
\newcommand{\relwithtext}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize#2}}}{#3}}%
}


\ifconf{}{
	\usepackage[
		amsmath,
		hyperref,
		thmmarks,
	]{ntheorem}
	
	\let\qed\relax
	
	\theorembodyfont{\slshape}
	\theoremseparator{:}
	\newtheoremstyle{proofstyle}%
	  {\item[\theorem@headerfont\hskip\labelsep ##1\theorem@separator]}%
	  {\item[\theorem@headerfont\hskip\labelsep ##1 ##3\theorem@separator]}
	
	%
	%
	\theorempreskip{\topsep} %
	%
	
	\newtheorem{theorem}{Theorem}[section]
	
	\theoremstyle{plain}
	\theorempreskip{\topsep}
	
	\newtheorem{proposition}[theorem]{Proposition}
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{conjecture}[theorem]{Conjecture}
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{definition}[theorem]{Definition}
	
	\theoremstyle{plain}
	\theorembodyfont{\upshape}
	
	\newtheorem{property}[theorem]{Property}
	\newtheorem{fact}[theorem]{Fact}
	
	%
	\theoremsymbol{\raisebox{-.25ex}{$\Box$}}
	\qedsymbol{\raisebox{-.25ex}{$\Box$}}
	
	
	\theoremstyle{proofstyle}
	\newtheorem{proof}{Proof}


%
%%
%
%
%
%
%
%
%
%
%
%
%%
%%
%

}

\newenvironment{thmenumerate}[1]{%
	\begin{enumerate}[
		label={\makebox[\widthof{(a)}][c]{\textup{(\alph*)}}},
		ref={\ref{#1}\kern.1em--\kern.1em(\alph*)},
		itemsep=0pt,
	]%
}{%
	\end{enumerate}%
}


%
%
\usepackage{tikz}
\tikzset{every picture/.style={/utils/exec={\sffamily}}}
\tikzoption{base font}{\def\tikz@base@textfont{#1}}
\tikzoption{font}{\def\tikz@textfont{\tikz@base@textfont#1}}
\tikzset{
  base font=\sffamily,
}
\usepackage{comment}
\tikzset{elegant/.style={domain=-2:2,thick,samples=201,magenta,line cap=rect,line join=bevel}}

\usetikzlibrary{calc,external}
%\tikzexternalize[mode=list and make]

\hypersetup{
%
%
%
%
	final,
	hidelinks,
	bookmarksnumbered=true,
	bookmarks=true,
	bookmarksopenlevel=2,
	bookmarksopen=true,
}
%
%



%%
%%
%%
\tolerance 1414
\hbadness 1414
\emergencystretch 1.5em	 %
\hfuzz 0.3pt	%
\vfuzz \hfuzz	

%%
\widowpenalty=10000
\clubpenalty=10000

%%
\raggedbottom

%%
%%
%%
\allowdisplaybreaks[3]



\setcounter{tocdepth}{2}

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{\vskip 0.2in
\noindent 
\begin{fminipage}{6.3in}
}{
\end{fminipage}
\vskip 0.2in
}

\def\pleq{\preccurlyeq}
\def\pgeq{\succcurlyeq}
\def\pge{\succ}
\def\ple{\prec}

\def\Approx#1{\approx_{#1}}

\def\Span#1{\textbf{Span}\left(#1  \right)}
\def\bvec#1{{\mbox{\boldmath $#1$}}}

\ifarxiv{
	\def\vec#1{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
	{\mbox{\boldmath$\textstyle#1$}}
	{\mbox{\boldmath$\scriptstyle#1$}}
	{\mbox{\boldmath$\scriptscriptstyle#1$}}}
}{}

\def\prob#1#2{\mbox{\normalfont{Pr}}_{#1}\left[ \normalfont{#2} \right]}
\def\pvec#1#2{\vec{\mbox{P}}^{#1}\left[ #2 \right]}
\def\expec#1#2{{\mathbb{E}}_{#1}\left[ #2 \right]}
\def\var#1{\mbox{\bf Var}\left[ #1 \right]}
\newcommand{\E}{\mbox{{\bf E}}}

\def\defeq{\stackrel{\mathrm{def}}{=}}
\def\setof#1{\left\{#1  \right\}}
\def\sizeof#1{\left|#1  \right|}

\def\floor#1{\left\lfloor #1 \right\rfloor}
\def\ceil#1{\left\lceil #1 \right\rceil}

\def\dim#1{\mathrm{dim} (#1)}
\def\sgn#1{\mathrm{sgn} (#1)}

\def\union{\cup}
\def\intersect{\cap}
\def\Union{\bigcup}
\def\Intersect{\bigcap}

\def\abs#1{\left|#1  \right|}

\def\norm#1{\left\| #1 \right\|}
\def\smallnorm#1{\| #1 \|}


\def\calC{\mathcal{C}}
\def\calE{\mathcal{E}}
\def\calG{\mathcal{G}}
\def\calL{\mathcal{L}}
\def\calS{\mathcal{S}}


\newcommand\Ppsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\PPsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\pphi{\boldsymbol{\mathit{\phi}}}
\newcommand\Llambda{\boldsymbol{\mathit{\Lambda}}}
\newcommand\PPi{\boldsymbol{\Pi}}

\newcommand\pa{\boldsymbol{\text{p}}}
\newcommand\ppi{\boldsymbol{\pi}}
\newcommand\cchi{\boldsymbol{\chi}}
\newcommand\aalpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\ggamma{\boldsymbol{\gamma}}
\newcommand\ddelta{\boldsymbol{\delta}}



\def\aa{\pmb{\mathit{a}}}
\newcommand\bb{\boldsymbol{\mathit{b}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\dd{\boldsymbol{\mathit{d}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
\renewcommand\gg{\boldsymbol{\mathit{g}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\jj{\boldsymbol{\mathit{j}}}
\newcommand\kk{\boldsymbol{\mathit{k}}}
\renewcommand\ll{\boldsymbol{\mathit{l}}}
\newcommand\pp{\boldsymbol{\mathit{p}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\bs{\boldsymbol{\mathit{s}}}
\newcommand\nn{\boldsymbol{\mathit{n}}}
\newcommand\rr{\boldsymbol{\mathit{r}}}
\renewcommand\ss{\boldsymbol{\mathit{s}}}
\def\tt{\boldsymbol{\mathit{t}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
\newcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\ww{\boldsymbol{\mathit{w}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}
\newcommand\xxbar{\overline{\boldsymbol{\mathit{x}}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\CC{\boldsymbol{\mathit{C}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\EE{\boldsymbol{\mathit{E}}}
\newcommand\GG{\boldsymbol{\mathit{G}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\KK{\boldsymbol{\mathit{K}}}
\newcommand\NN{\boldsymbol{\mathit{N}}}
\newcommand\MM{\boldsymbol{\mathit{M}}}
%
\newcommand\PP{\boldsymbol{\mathit{P}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\UU{\boldsymbol{\mathit{U}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\VV{\boldsymbol{\mathit{V}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\newcommand\YY{\boldsymbol{\mathit{Y}}}
\newcommand\ZZ{\boldsymbol{\mathit{Z}}}


\newcommand\sink{v_\textnormal{sink}}
\newcommand\Path[1]{\textsc{Path}_{#1}}
\renewcommand\line{\textsc{Line}}
\renewcommand\square[1]{\textsc{Square}_{#1}}
\newcommand\cube[1]{\text{$d$-}\textsc{Cube}_{#1}}
\newcommand\Otil{\widetilde{O}}

\newcommand\xhat{\boldsymbol{\hat{\mathit{x}}}}
\newcommand\uhat{{\hat{{u}}}}
\newcommand\vhat{{\hat{{v}}}}
\newcommand\what{{\hat{{w}}}}

\newcommand\ttau{\boldsymbol{\mathit{\tau}}}

\newcommand{\sym}[1]{\mathrm{sym} (#1)}

\renewcommand{\deg}[1]{\text{deg}(#1)}
\newcommand{\er}{\mathcal{R}_{\textnormal{eff}}}

%

\newcommand{\polylog}{\text{polylog}}
\newcommand{\etal}{~\textit{et. al.}}


\newcommand{\rp}[1]{{\bf \color{green} Richard: #1}}
\newcommand{\yu}[1]{{\bf \color{magenta} Yu: #1}}
\newcommand{\david}[1]{{\bf \color{blue} David: #1}}
\newcommand{\ar}[1]{{\bf \color{cyan} Anup: #1}}

%%
%%

\newcommand{\solutionset}{\mathcal S}%
\newcommand{\solutionsettrunc}[1]{\mathcal S_{#1}}%

\newcommand{\polytope}{+\textsc{sloped}}

\newcommand{\upperhull}{\textsc{u-hull}}%

\newcommand{\lowerhull}{\textsc{l-hull}}%

\newcommand{\urhull}{\textsc{upper-right-hull}}

\newcommand{\llhull}{\textsc{lower-left-hull}}

\newcommand\sndOrdOnlyP[1][i]{%
	P_{#1}^{\vphantom{\scriptscriptstyle g}\smash{\scriptscriptstyle(}z\smash{\scriptscriptstyle)}}
}

\newcommand{\UR}{\textsc{URHULL}}
\newcommand{\UL}{\textsc{ULHULL}}
\newcommand{\LL}{\textsc{LLHULL}}
\newcommand{\LR}{\textsc{LRHULL}}
\newcommand{\ed}{\simeq}


%
\makeatletter
\let\@@pmod\pmod
\DeclareRobustCommand{\pmod}{\@ifstar\@pmods\@@pmod}
\def\@pmods#1{\mkern4mu({\operator@font mod}\mkern 6mu#1)}
\makeatother

\newcommand{\FullVersion}[1]{#1}

%
%
%
%
%

\let\epsilon\varepsilon

